Incremental Verification of Neural Networks

Complete verification of deep neural networks (DNNs) can exactly determine whether the DNN satisfies a desired trustworthy property (e.g., robustness, fairness) on an infinite set of inputs or not. Despite the tremendous progress to improve the scalability of complete verifiers over the years on individual DNNs, they are inherently inefficient when a deployed DNN is updated to improve its inference speed or accuracy. The inefficiency is because the expensive verifier needs to be run from scratch on the updated DNN. To improve efficiency, we propose a new, general framework for incremental and complete DNN verification based on the design of novel theory, data structure, and algorithms. Our contributions implemented in a tool named IVAN yield an overall geometric mean speedup of 2.4x for verifying challenging MNIST and CIFAR10 classifiers and a geometric mean speedup of 3.8x for the ACAS-XU classifiers over the state-of-the-art baselines.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Paper/Theorems/theorem0a.tex <==
\begin{restatable}{theorem}{timebab}(Time Complexity of BaB).
\label{theorem:timebab} For BaB that starts from scratch halts with the final specification tree $T$, $\Time{T} = \tbr \cdot (|\nodes{T}| - |\leaves{T}|) + \tbo \cdot |\nodes{T}|$. 
\end{restatable}


==> Paper/Theorems/theorem0b.tex <==
\begin{proof}
For BaB verification that generates a tree $T$, the branching call is made for each internal node of the tree. $\nodes{T}/\leaves{T}$ is the set of internal nodes of the tree. Therefore, this takes a total $\tbr \cdot (|\nodes{T}| - |\leaves{T}|)$ time. The analyzer call is made for each node of the tree, and therefore, it takes a total of $\tbo \cdot |\nodes{T}|$ time. With our simplification we have $\Time{T} = \tbr \cdot (|\nodes{T}| - |\leaves{T}|) + \tbo \cdot |\nodes{T}|$.
\end{proof}

==> Paper/Theorems/theorem1a.tex <==
\begin{restatable}{theorem}{bestreuse}(Best Case Complexity of Reuse).
\label{theorem:bestreuse} Given incremental verifier $V_\Delta$, $\Tinit = T^{N}_{f}$ then $\Timeb(\Tinit,  T^{\perturbedNetwork}_f) \geq  \frac{\tbo \cdot (|\nodes{T^{N}_{f}}|+1)}{2}$ with $T^{\perturbedNetwork}_{f}$ as the final tree and the $\ver$ as the output in verifying $\perturbedNetwork$.  
\end{restatable}


==> Paper/Theorems/theorem1b.tex <==
\begin{proof}
For a full binary tree $|\leaves{T^{N}_{f}}| = \frac{|\nodes{T^{N}_{f}}|+1}{2}$. 
\begin{align*}
     & |\nodes{T^{\perturbedNetwork}_f}| \geq |\nodes{\Tinit}| && \text{(Since $T^{\perturbedNetwork}_f > \Tinit$)}\\
    & \Timeb(\Tinit,  T^{\perturbedNetwork}_f) \geq |\leaves{T^{N}_{f}}| && \text{(From Theorem~\ref{thm:timeinc}}\\
   & \Timeb(\Tinit,  T^{\perturbedNetwork}_f) \geq \frac{|\nodes{T^{N}_{f}}|+1}{2}\\
\end{align*}
\end{proof}

==> Paper/Theorems/theorem5a.tex <==
% \begin{restatable}{theorem}{provepreservation}
% \label{thm:prove_preservation}
% If $\EpsNorm \leq \frac{|\ProblemMin(\FeasibleReg(\OrgNetwork_{\Layers}, T))|}{\|\Lpc\|_2 \cdot \MaxNorm(N_{\Layers}, T)}$ then for any pertrubed network $\perturbedNetwork \in \mathcal{M}(N, \EpsNorm)$, $\SolvFunc(\OrgNetwork, T) \implies \SolvFunc(\perturbedNetwork, T)$.
% \end{restatable}

==> Paper/Theorems/theorem5b.tex <==
\begin{proof}
We prove this by contradiction. Suppose $\ProblemMin(\perturbedNetwork, T) < 0$ then $\exists Y' \in \FeasibleReg(\perturbedNetwork, T)$ such that $\Lpc^{T}Y' < 0$. 
Swapping $\OrgNetwork$ with $\perturbedNetwork$ in lemma~\ref{lem:feasible_solution} we can show $Y \in \FeasibleReg(\OrgNetwork, T)$ such that $\|Y - Y'\|_2 \leq \EpsNorm \cdot \MaxNorm(\FeasibleReg(\perturbedNetwork, T))$. 
Given perturbation is done only at the final layer $\forall i \in [\Layers - 1]$ $\OrgNetwork_{i} = \perturbedNetwork_{i}$ which implies $\MaxNorm(\OrgNetwork, T, \Layers - 1) = \MaxNorm(\perturbedNetwork, T, \Layers-1)$. 
As $Y \in \FeasibleReg(\OrgNetwork, T)$ then $\Lpc^Ty \geq \ProblemMin(\FeasibleReg(\OrgNetwork, T))$. 
\begin{equation*}
    \begin{split}
        \Lpc^{T} Y' &= \Lpc^T Y + \Lpc^{T}(Y' - Y)
             &\geq \Lpc^T Y - \|\Lpc\|_2\|(Y' - Y)\|_2 \\
             &\geq \Lpc^T Y - \|\Lpc\|_2 \cdot \EpsNorm \cdot \MaxNorm(\OrgNetwork, T, \Layers - 1) \\
             &\geq \ProblemMin(\FeasibleReg(\OrgNetwork, T))  - |\ProblemMin(\FeasibleReg(\OrgNetwork, T))| \geq 0\;\; \text{given}\;\;\ProblemMin(\FeasibleReg(\OrgNetwork, T)) \geq 0 
    \end{split}
\end{equation*}
The above derivation shows that $\Lpc^TY' \geq 0$ which contradicts the assumptions that $\Lpc^TY' < 0$ and $\ProblemMin(\FeasibleReg(\perturbedNetwork, T)) < 0$. Hence if the given condition holds then we can use the same specification tree $T$ for proving the property on any perturbed network $\perturbedNetwork$ sampled from $\EpsNorm \leq \frac{|\ProblemMin(\FeasibleReg(\OrgNetwork, T))|}{\|\Lpc\|_2 \cdot \MaxNorm(N, T, \Layers - 1)}$. 
\end{proof}

==> Paper/images/speedup.tex <==
\begin{tikzpicture}
  \begin{axis}[
    label style={font=\large},
    tick label style={font=\Large},
    xlabel={\static{} Speedup (over \elina{})},
    x label style={at={(axis description cs:0.5,-0.025)}, anchor=north},
    xtick style={draw=none},
    xmin=-8,
    xmax=12,
    xtick={-8, -4, 0, 4, 8, 12},
    xticklabels={$2^{-8}$, $2^{-4}$, $1$, $2^4$, $2^8$, $2^{12}$},
    ylabel={\static{} Precision (\%)},
    y label style={at={(axis description cs:0.025,0.79)}, anchor=east},
    ytick style={draw=none},
    ymin=0,
    ymax=100,
    ytick={0, 20, 40, 60, 80, 100},
    yticklabels={0, 20, 40, 60, 80, 100},
    scatter/classes={
      ld_finished={mark=x, draw=scatterblue, mark size=3},
      ld_to={mark=x, draw=scatterred, mark size=3}
    }
  ]
    \addplot[scatter, only marks, scatter src=explicit symbolic]
    table[meta=label] {
      x y label
      0.07682967088470205 81.5556590591523 ld_finished
      0.05554255972405288 81.32837900603809 ld_finished
      0.07666878067347214 81.44186046511628 ld_finished
      0.043624815752270306 100.0 ld_finished
      0.20988051879580566 99.23053711526856 ld_finished
      0.019296948810188425 97.9750107712193 ld_finished
      0.07491114556011048 77.23656122647002 ld_finished
      0.05776111817547789 100.0 ld_finished
      2.501486138155239 95.09163142381135 ld_finished
      0.06239541323942857 97.05150296764312 ld_finished
      0.10104401257033603 98.89990493005568 ld_finished
      0.19910480930271782 94.21067495057893 ld_finished
      0.007881776111809145 76.18694362017804 ld_finished
      0.022080167608587286 76.22222222222223 ld_finished
      0.0934420117270459 33.78517754530721 ld_finished
      2.1986905172082403 95.0427129174217 ld_finished
      0.37359535330320315 28.35820895522388 ld_finished
      0.023705242339184782 100.0 ld_finished
      0.2821100980541862 67.02448842670245 ld_finished
      0.1808252931142122 72.77306468716861 ld_finished
      0.24880007819516978 98.70941722121395 ld_finished
      0.0014845810195280474 95.99164926931107 ld_finished
      -0.010553791935000728 95.56356795736008 ld_finished
      0.05553395302297589 94.74028095393662 ld_finished
      0.03005884506017024 98.77966101694915 ld_finished
      0.011048618739811033 96.10963748894783 ld_finished
      0.44467308467753164 89.20152091254752 ld_finished
      4.413184737043818 91.87566231013776 ld_finished
      1.3707589039721415 83.1715210355987 ld_finished
      3.4265677408618336 59.001782531194294 ld_finished
      -0.05137693145335606 18.88341543513957 ld_finished
      -0.10891221142221556 34.439311213775724 ld_finished
      -0.016931784786597636 20.235934664246823 ld_finished
      0.02317094649326859 95.8049214349244 ld_finished
      0.1273721662846366 85.44373486016296 ld_finished
      0.07310516516210384 100.0 ld_finished
      -0.13184463727072834 98.97555296856811 ld_finished
      0.20615107430018204 70.36090705844778 ld_finished
      0.13054824181657157 98.73542778107094 ld_finished
      0.17101010157072452 97.40103958416634 ld_finished
      -0.058104325167465616 85.13761467889908 ld_finished
      0.22198666870376763 100.0 ld_finished
      0.29736198489404236 98.14974182444061 ld_finished
      9.731634923621742 86.07888631090486 ld_finished
      -1.1296520045040348 64.90066225165563 ld_finished
      5.238373462755775 100.0 ld_finished
      4.703303114551094 98.88789237668162 ld_finished
      0.09477374184071448 99.950137122912 ld_finished
      -0.1360039062850432 99.95021160069703 ld_finished
      5.621773543601076 98.9213639526792 ld_finished
      -0.11351783521035066 99.96449494052902 ld_finished
      4.568331011868031 98.87823412339425 ld_finished
      1.4583664700809595 66.42011834319527 ld_finished
      3.922017159492751 97.32441471571906 ld_finished
      -0.121419350811814 99.95021160069703 ld_finished
      4.423715952343999 98.81588999236058 ld_finished
      1.1870534078924673 60.82910321489001 ld_finished
      -0.21064581179901828 93.82089046893516 ld_finished
      -0.05980184099402284 96.2830887395419 ld_finished
      -0.20021108874525945 95.71801566579634 ld_finished
      0.06595841540299159 96.26321974148061 ld_finished
      0.02966574406538203 95.83685545224007 ld_finished
      0.04695328734209586 99.06815274986296 ld_finished
      -0.32288015992736735 97.1375464684015 ld_finished
      0.14243256228987605 96.23558827614946 ld_finished
      -0.02315220059987339 95.06059493206023 ld_finished
      0.04419265422402147 96.6875 ld_finished
      0.3498056205836034 99.06917320678956 ld_finished
      -0.09311120838153171 97.14073523950985 ld_finished
      0.029886574642651362 96.23872310895212 ld_finished
      0.13487534945236332 95.74247144340602 ld_finished
      0.09154789077022153 100.0 ld_finished
      -0.03136340130800339 100.0 ld_finished
      0.2594299931885983 98.87904538058217 ld_finished
      -0.00983140942542199 97.35349716446125 ld_finished
      -0.0010682790202102002 97.09819038440946 ld_finished
      -0.024785436860034534 95.71355236139631 ld_finished
      0.2052534100971172 96.36405213812029 ld_finished
      0.17109056500711253 100.0 ld_finished
      0.09030434554933892 95.87779870265746 ld_finished
      0.13422727886434746 99.07775768535262 ld_finished
      0.5115031245810487 98.76346230554448 ld_finished
      -0.19272531996672215 97.16651333946642 ld_finished
      0.11815946692100233 96.28716262501713 ld_finished
      8.348722859571419 80.84615384615384 ld_finished
      -0.27197058198569524 100.0 ld_finished
      -0.05480003075726738 85.49434688477268 ld_finished
      3.132687142942452 82.90830168204015 ld_finished
      -0.19510118900734197 75.93984962406014 ld_finished
      -0.1534623481701925 100.0 ld_finished
      0.28267300758781005 100.0 ld_finished
      0.06772330026300726 94.5945945945946 ld_finished
      0.07514708571588796 55.76470588235294 ld_finished
      -0.2453410732705594 100.0 ld_finished
      -0.018972042424575418 100.0 ld_finished
      0.1389797296229614 97.89653212052303 ld_finished
      -0.33628568739103143 100.0 ld_finished
      0.010319923562873074 98.77358490566037 ld_finished
      -0.2791805964473788 84.17462482946793 ld_finished
      -0.13611675803604595 98.04469273743017 ld_finished
      0.3353156855937482 100.0 ld_finished
      -0.48671929826964244 100.0 ld_finished
      0.1528850482399928 100.0 ld_finished
      -0.05583618610249541 100.0 ld_finished
      -0.12502034355768782 100.0 ld_finished
      -0.19284762561015578 95.31502423263328 ld_finished
      0.02409735018919582 53.95061728395062 ld_finished
      0.11325109001172684 100.0 ld_finished
      -1.5016333597120661 94.52054794520548 ld_finished
      0.45324988396901456 100.0 ld_finished
      2.33790709520269 95.04335447133428 ld_finished
      -0.00953707300061475 99.62942629700797 ld_finished
      -0.12229987490482157 81.9672131147541 ld_finished
      0.2089345895516436 94.98525073746312 ld_finished
      0.2522162189483962 98.98078043098427 ld_finished
      0.1319414352610026 100.0 ld_finished
      0.020548068449818498 68.79502292075966 ld_finished
      -0.03218657123893268 99.07658016239452 ld_finished
      0.31041793663773576 100.0 ld_finished
      -0.2805650300966213 98.84311179317672 ld_finished
      0.5157371594859562 95.09976525821597 ld_finished
      -0.08594285048238919 95.25631216526396 ld_finished
      0.20153705743126246 97.18647764449291 ld_finished
      -0.12472680984234645 100.0 ld_finished
      0.045191399685088486 97.11394302848576 ld_finished
      -0.3353748955689103 97.42996063903682 ld_finished
      0.33380854453191117 29.075425790754256 ld_finished
      -0.06272111108065744 32.04376709652208 ld_finished
      0.2268309649200437 91.11316113161132 ld_finished
      0.018090884619229242 97.11394302848576 ld_finished
      -6.813527217967391 63.46456692913386 ld_finished
      0.08939564818584649 92.12291374200593 ld_finished
      7.350827845726082 95.0957496496964 ld_finished
      -6.659300594165744 61.12696148359487 ld_finished
      0.052604157665958766 98.68538990140424 ld_finished
      -0.27415828949328785 94.02053712480253 ld_finished
      3.630096588709813 90.36334913112164 ld_finished
      0.027430531610979338 100.0 ld_finished
      0.11360535838063028 88.62395340371314 ld_finished
      0.2160127026310531 98.97564746810978 ld_finished
      -0.06169639440409803 100.0 ld_finished
      -0.04324398437561972 97.89259007477906 ld_finished
      0.7638634243611567 91.90022421524664 ld_finished
      0.0009494797708443045 95.09841759938247 ld_finished
      -0.11464421200864337 100.0 ld_finished
      7.975358174292285 79.08771929824562 ld_finished
      7.934198492491814 79.55375253549695 ld_finished
    };
  \end{axis}
\end{tikzpicture}

==> Paper/technical/time_complexity.tex <==
\subsection{Time complexity of verification:}
\label{sec:complexity}

We next state the best-case complexity of the reuse technique when $V_\Delta$ output is $\ver$. \fTBD{Why is best time improtant? Also what about the worst time?}
\input{Theorems/theorem1a.tex}
The best case complexity when $V_\Delta$ output is $\counterex$ is trivial $\tbo$. Since it is possible that the first node of $\Tinit$ that the analyzer analyzes finds a counterexample.\fTBD{What do we gain by this statement? How does it connect with the full Algo1? I see now you use in the next section.. but then make it a corolary and reference directly there...}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

